On the Sparse DAG Structure Learning Based on Adaptive Lasso

Learning the underlying Bayesian Networks (BNs), represented by directed acyclic graphs (DAGs), of the concerned events from purely-observational data is a crucial part of evidential reasoning. This task remains challenging due to the large and discrete search space. A recent flurry of developments followed NOTEARS[1] recast this combinatorial problem into a continuous optimization problem by leveraging an algebraic equality characterization of acyclicity. However, the continuous optimization methods suffer from obtaining non-spare graphs after the numerical optimization, which leads to the inflexibility to rule out the potentially cycle-inducing edges or false discovery edges with small values. To address this issue, in this paper, we develop a completely data-driven DAG structure learning method without a predefined value to post-threshold small values. We name our method NOTEARS with adaptive Lasso (NOTEARS-AL), which is achieved by applying the adaptive penalty method to ensure the sparsity of the estimated DAG. Moreover, we show that NOTEARS-AL also inherits the oracle properties under some specific conditions. Extensive experiments on both synthetic and a real-world dataset demonstrate that our method consistently outperforms NOTEARS.

==> Pages/Appendices/Further_evaluations.tex <==
\section{Further Evaluations}
Figure~\ref{fig7} and Figure~\ref{fig8} show structure recovery results for SEM with exponential noise and gumbel noise respectively, where the weights of existing edges are sampled from a normal distribution with mean $0$ and variance $2^2$. 
\begin{figure}[!t]
	\centering
	\includegraphics[width=\columnwidth]{Figures/exp_ER_gausswei.pdf} 
	\caption{Numerical results in terms of SHD, TPR and FDR on ER graphs, with sample size $n = 1000$ and Exponential noise.}
	\label{fig7}
\end{figure}

\begin{figure}[!t]
	\centering
	\includegraphics[width=\columnwidth]{Figures/gumbel_ER_gausswei.pdf} 
	\caption{Numerical results in terms of SHD, TPR and FDR on ER graphs, with sample size $n = 1000$ and Gumbel noise.}
	\label{fig8}
\end{figure}

